ForeAct3D: Policy-Grounded Future World Modeling for VLA Policies

Robots need to anticipate how their actions will change the world, since manipulation success hinges on the resulting contacts and object motions. However, existing Vision-Language-Action (VLA) policies that predict future observations from shared features leave the forecast decoupled from the actions the policy will actually execute, and impose no physical constraints on how the scene may evolve. We introduce ForeAct3D, a framework for policy-grounded future world modeling within VLA policies. Learnable geometric queries decode depth, semantic segmentation, and camera pose from the policy representation into current and future semantic 3D scene states, and the future queries are conditioned on the policy-generated action chunk to ground the forecast in the planned interaction. A physical-consistency closure relates the two states through background staticity and instance-level rigidity, and anchors the wrist-camera pose to end-effector kinematics. These objectives shape the shared representation used for action generation during training, and no future prediction is required at inference. Without robot pretraining, ForeAct3D achieves 98.3% average success on LIBERO and an average task length of 3.73 on CALVIN, outperforming its base policy on every suite. Ablations show that semantic 3D supervision, physical consistency, and action conditioning each improve manipulation performance, and that action conditioning substantially improves future object localization. Real-world experiments on spatial placement, object insertion, and sequential manipulation further raise average success from 6.7% to 37.8% over the base policy. The project page and code are available at https://github.com/anthonytao80-crypto/ForeAct3D.

==> tab/action_condition.tex <==
\begin{table}[!htbp]
\centering
\caption{Effect of action conditioning on future depth-derived geometry on CALVIN. Both variants use the same evaluation protocol and prediction horizon of $T=8$.}
\label{tab:action_conditioning_full}
\begin{tabular}{lcc}
\toprule
Metric & ForeAct3D & w/o Action Conditioning \\
\midrule
AbsRel $\downarrow$ & 0.0117 & 0.0165 \\
RMSE (m) $\downarrow$ & 0.1633 & 0.2144 \\
$\delta_1$ $\uparrow$ & 0.9933 & 0.9881 \\
Scene CD (m) $\downarrow$ & 0.0206 & 0.0220 \\
Scene EMD (m) $\downarrow$ & 0.0623 & 0.0655 \\
Inst-CD (m) $\downarrow$ & 0.0137 & 0.0183 \\
Trans (cm) $\downarrow$ & 1.25 & 1.77 \\
Recall@2cm $\uparrow$ & 0.928 & 0.799 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/geometry_full.tex <==
\begin{table}[t]
\centering\footnotesize
\caption{\textbf{Complete depth-derived geometry on CALVIN.} Instance metrics use GT masks. Rows separate current and future states; future horizons are 5 (CLOVER), 3 (DreamVLA), and 8 (ForeAct3D). Depth RMSE, CD, and EMD use meters; translation uses centimeters; recall is a fraction.}
\label{tab:geometry_full}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}llrrrrrrrr@{}}
\toprule
& & \multicolumn{3}{c}{Depth} & \multicolumn{2}{c}{Scene} & \multicolumn{3}{c}{GT instance regions} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-7}\cmidrule(lr){8-10}
Method & State & AbsRel & RMSE & $\delta_1$ & CD & EMD & Inst-CD & Trans & Recall \\
\midrule
CLOVER & Future & 0.0083 & 0.1252 & 0.9955 & 0.0195 & 0.0601 & 0.0139 & 1.741 & 0.7582 \\
DreamVLA & Future & 0.0867 & 0.5583 & 0.9126 & 0.1350 & 0.3145 & 0.1455 & 20.61 & 0.1073 \\
ForeAct3D & Current & 0.0110 & 0.1551 & 0.9942 & 0.0206 & 0.0631 & 0.0129 & 1.165 & 0.9416 \\
ForeAct3D & Future & 0.0117 & 0.1633 & 0.9933 & 0.0206 & 0.0623 & 0.01371 & 1.245 & 0.9278 \\
\bottomrule
\end{tabular}
\end{table}


==> tab/libero_action_details.tex <==
\begin{table}[htbp]
\centering
\small
\caption{\textbf{Action-conditioning results by LIBERO suite.} Values are measured at the future prediction horizon under the same GT-mask protocol as Table~\ref{tab:semantic_localization}. Full denotes ForeAct3D with action conditioning; w/o action denotes the variant without it. The main-text instance metrics are equal-weight averages of the four suites, computed before rounding.}
\label{tab:libero_action_details}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{@{}llrrrrrr@{}}
\toprule
Suite & Variant & AbsRel $\downarrow$ & RMSE $\downarrow$ & $\delta_1$ $\uparrow$ & Inst-CD $\downarrow$ & Trans $\downarrow$ & Recall $\uparrow$ \\
& & & (m) & & (m) & (cm) & @2cm \\
\midrule
\multirow{2}{*}{Goal} & Full & 0.0225 & 0.214 & 0.976 & 0.0101 & 1.58 & 0.912 \\
 & w/o action & 0.0562 & 0.315 & 0.945 & 0.0126 & 2.65 & 0.879 \\
\midrule
\multirow{2}{*}{Object} & Full & 0.0078 & 0.067 & 0.994 & 0.0068 & 0.56 & 0.967 \\
 & w/o action & 0.0388 & 0.216 & 0.958 & 0.0115 & 2.82 & 0.908 \\
\midrule
\multirow{2}{*}{Spatial} & Full & 0.0229 & 0.230 & 0.973 & 0.0076 & 0.71 & 0.957 \\
 & w/o action & 0.0769 & 0.378 & 0.929 & 0.0123 & 2.33 & 0.880 \\
\midrule
\multirow{2}{*}{LIBERO-10} & Full & 0.0173 & 0.095 & 0.987 & 0.0105 & 1.38 & 0.924 \\
 & w/o action & 0.0598 & 0.224 & 0.951 & 0.0133 & 2.55 & 0.869 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/semantic_localization.tex <==
\begin{table}[!htbp]
\centering\small
\caption{\textbf{Future localization with predicted depth and semantic masks.} GT instance IDs are retained in both mask settings. Recall@2cm is in percent. These results assess localization with predicted semantic support, not autonomous instance detection without GT IDs.}
\label{tab:semantic_localization}
\begin{tabular}{@{}llrrrr@{}}
\toprule
& & \multicolumn{2}{c}{Trans (cm) $\downarrow$} & \multicolumn{2}{c}{Recall@2cm $\uparrow$} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
Benchmark & Suite & GT mask & Pred mask & GT mask & Pred mask \\
\midrule
LIBERO & Object & 0.56 & 0.48 & 96.7 & 96.9 \\
& Goal & 1.58 & 1.20 & 91.2 & 92.8 \\
& Spatial & 0.71 & 0.67 & 95.7 & 96.3 \\
& Long & 1.38 & 1.13 & 92.4 & 93.8 \\
& Average & 1.06 & 0.87 & 94.0 & 94.9 \\
\midrule
CALVIN & ABC$\rightarrow$D & 1.25 & 3.49 & 92.8 & 65.9 \\
\bottomrule
\end{tabular}
\end{table}

==> tab/semantic_quality.tex <==
\begin{table}[t]
\centering\small
\caption{\textbf{Three-class semantic segmentation quality (\%).} Future class IoUs are reported for background, robot, and object. All objects share the same semantic class. LIBERO Average denotes the mean across the Object, Goal, Spatial, and Long task suites.}
\label{tab:semantic_quality}
\begin{tabular}{@{}llrrrrr@{}}
\toprule
Benchmark & Suite & mIoU@$t$ & BG@$t+T$ & Robot@$t+T$ & Object@$t+T$ & mIoU@$t+T$ \\
\midrule
LIBERO & Object & 98.0 & 99.4 & 95.8 & 98.0 & 97.7 \\
& Goal & 87.2 & 94.8 & 94.8 & 70.8 & 86.8 \\
& Spatial & 78.1 & 91.5 & 95.7 & 45.7 & 77.6 \\
& Long & 93.7 & 97.2 & 94.5 & 87.8 & 93.2 \\
& Average & 89.3 & 95.7 & 95.2 & 75.6 & 88.8 \\
\midrule
CALVIN & ABC$\rightarrow$D & 88.0 & 89.8 & 90.3 & 77.3 & 85.8 \\
\bottomrule
\end{tabular}
\end{table}
